The CARMENES search for exoplanets around M dwarfs. Revisiting the GJ 581 multi-planetary system with new Doppler measurements from CARMENES, HARPS, and HIRES

GJ 581 is a nearby M dwarf known to host a packed multiple planet system with 2 super-Earths and a Neptune-mass planet. We present new orbital analyses of the system, utilizing recent RV data obtained from the CARMENES spectrograph combined with newly reprocessed archival data from the HARPS and HIRES spectrographs. Our aim was to analyze the post-discovery spectroscopic data of GJ 581, which were obtained with CARMENES. In addition, we used publicly available HIRES and HARPS spectroscopic data to seek evidence of the known and disputed exoplanets in this system. We aimed to investigate the stellar activity of GJ 581 and update the planetary system's orbital parameters using state-of-the-art numerical models and techniques. We performed a periodogram analysis of the available precise CARMENES, HIRES, and HARPS RVs and of stellar activity indicators. We conducted detailed orbital analyses by testing various orbital configurations consistent with the RV data. We studied the posterior probability distribution of the parameters fit to the data and explored the long-term stability and overall orbital dynamics of the system. We refined the orbital parameters of the system using the most precise and complete set of Doppler data available. Consistent with the existing literature, we confirm that the system is unequivocally composed of only 3 planets detectable in the present data, dismissing the putative planet GJ 581 d as an artifact of stellar activity. Our N-body fit reveals that the system's inclination is i $=$ 47.0 deg, which implies that the planets could be up to 30% more massive than their previously reported minimum masses. Furthermore, we report that the system exhibits long-term stability, as indicated by the posterior probability distribution, characterized by secular dynamical interactions without the involvement of mean motion resonances.

==> referee_report.tex <==
Dear Editor,
 
 

We extend our sincere gratitude to the referee for reviewing our manuscript. We greatly appreciate the positive and constructive feedback provided in the referee report, which has contributed to improving our work.

 
 
#####################################################################################
Reviewer:


This is a report on "The CARMENES search for exoplanets around M dwarfs: Revisiting the GJ 581 multi-planetary system with new Doppler measurements from CARMENES, HARPS, and HIRES." The manuscript presents new precise RV measurements of the historically and scientifically significant GJ 581 exoplanet system. It also describes dynamical modeling to the data that constrains the orbital inclination--and hence true masses--of the planetary orbits, which is rare for a non-transiting system of small planets. The data and analysis are sufficiently compelling to merit publication, and the manuscript is generally well written. I have some minor comments I would encourage the authors to consider before the manuscript is published. Below, I have described my primary concern first, with less important remarks listed in the order in which they appear in the text.



Answer: We are grateful for the positive feedback! We have thoroughly reviewed all the comments and incorporated the suggested changes into the manuscript. Please find our detailed responses to each point below.

#####################################################################################

PRIMARY CONCERN

I appreciate the posterior corner plots presented for the model fits, but believe the priors should also be cataloged. In particular, I am curious about the GP activity model in the RV model. The best-fit value for the "GP period" is near 66 days--that of the false-positive planet d--but the true stellar rotation period appears to be solidly confirmed to be twice that period. Does the period prior allow the model to choose between the period or the first harmonic? Is the outcome of the modeling sensitive to that choice?

Answer: We thank the referee for this note. Indeed, we should have provided a table with 
the adopted priors in our NS scheme. Such a table is now listed in the appendix. 
Our preliminary numerical setup included a wide range of uniform priors to scan the parameter 
landscape. For the GP rot. period, in particular, we adopted a period range between 1 and 300 
days, which allows the GP to cover the stellar rotation period. Posteriors of this parameter 
had firmly converged to a period of ~67 days with a small uncertainty of +/- 1.3 days, which 
was not surprising given that this period coincides with the strong HARPS RV signal of the 
putative planet d. Consequently, for the final numerical configuration detailed in this study, 
we opted for a more focused Gaussian prior to the GP rotation period with parameters $\mu$ = 
66.7 d, $\sigma$ = 10 d, a choice we find very adequate. 


#####################################################################################
OTHER NOTES

1. In section 3.1, the characterization of Keck/HIRES as having a 3 m/s noise floor is an outdated description of that instrument's performance. 25 years of instrument and pipeline optimization have resulted in a noise floor closer to 1-2 m/s for bright stars, as evidenced by, e.g., Luhn et al. (2020, AJ, 159, 235). This number is more consistent with the quoted median uncertainties for the HIRES RVs of GJ 581.


Answer: The referee is, of course, right! We thank you for this note. We have corrected this statement, and we now added Luhn et al. (2020) and Butler et al. (2017) as references to the current HIRES precision.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

2. The TESS lightcurve analysis suggests the presence of periodic dimming near the period of the 3-day planet. The authors state that this signal cannot be consistent with transits of the planet unless we consider TTVs that are not expected from the known 3-planet system. Have the authors considered the presence of new planets? Specifically, the TLS spectrum in Figure 6 shows peaks near 0.75 days that exceed the three horizontal threshold lines (which are not well described). Could those peaks represent a new planet, and if so, could that planet induce TTVs on planet e that would explain the RV and photometric data?

Answer: We value the referee's insightful observation! Throughout our analysis, we thoroughly 
explored alternative possibilities, including periods such as 3.12 days and its 1-day alias 
(~0.76 days), where close frequencies were identified in the TLS periodogram. Despite these 
investigations, satisfactory convergence was not achieved when utilizing multi-Keplerian or 
photodynamical schemes.

As explained in the text, we did not find significant periods following a more meticulous PLD light curve analysis of the TESS 
data. Consequently, we concluded that although 
intriguing, these signals are likely false positives. Thus, we opted not to elaborate further on this aspect to maintain conciseness and focus within the paper. Nonetheless, recognizing that readers may have similar questions, we briefly explain our unsuccessful tests.


~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

3. The caption to Figure 7 includes some inconsistencies. The first sentence (and the y-axis) states that the periodogram shown is an MLP power spectrum, but the last sentence states it is a GLS. Additionally, the description of the colors/shapes used for the instrument markers is inconsistent with what is shown in the plot.

Answer: Fixed. The bottom Figure was initially a GLS periodogram, however, it has been adjusted to be an MLP periodogram and relevant mentions are adjusted to MLP (i.e. the caption of Figure 7.)

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

4. The third paragraph of section 5.2 states "From model 0 to 3, all three of the quality assessment values increased significantly. This outcome was expected as all three planets are confirmed, and injecting their signals should improve the statistical significance of the model." I suggest using a word other than "injecting," as that word is often used to describe the introduction of an artificial signal for sensitivity testing, as in an "injection-recovery test."

Answer: Fixed.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

5. Also in section 5.2, why does the inclination prior start at 10 degrees?

Answer:  We acknowledge that our prior selection could have been more explicitly articulated. 
We have now clarified our reasoning in the text. While recognizing that a uniform prior in 
cos(i) between 0 and 1 could have yielded similar outcomes; we opted for a 10-90 degree prior, 
based on our initial experimental setup (see, e.g., our answer in PRIMARY CONCERN) before we 
run our final NS test, which is demonstrated to be appropriate, as can be seen from the 
posterior probability distribution of Fig 8. 

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

6. Several places in the manuscript, it is speculated that the 66-day signal does not appear in the CARMENES RVs because 1) CARMENES has fewer RVs, and 2) the red waveband of CARMENES suppresses starspot signals. Nevertheless, I would be somewhat surprised that no trace of the signal appears in CARMENES if its amplitude were constant in time. It is perhaps worth remarking that the rotation period--which appears quite clearly in, say, HARPS H-alpha, is also completely absent in the CARMENES activity tracer periodograms. Perhaps GJ 581 was simply in a quiet phase during CARMENES observations, which further suppressed the 66-day signal?

Answer: We acknowledge this excellent remark. We added the accurate referee's insights to the text. We also point out in section 4.3 that these quiet periods may be possible, based on results found in Figure 2. Therefore this fits in well with the referee's suggestion. 


#####################################################################################
 

